The KV-Surgeon: Compensation-Aware Offline KV-Cache Compaction

Offline compaction of the key--value cache (KV-cache) reduces the cost of repeatedly querying a fixed context by constructing a smaller cache once and reusing it subsequently. The central challenge of compaction is deciding which cache entries to delete and which to retain. Existing methods score each candidate for deletion on its own, with the rest of the cache being held fixed. However, softmax renormalization of the attention operation couples these decisions in a nonlinear manner: removing one entry changes the attention weights of every remaining one. In this work, we introduce KV-Surgeon, which uses calibration data to take interactions into account in a tractable way. We derive a quadratic surrogate that admits closed-form expressions for jointly making the optimal greedy removal decision as well as compensation within the remaining entries. On QuALITY, LongHealth, and Long Code Arena, and at every evaluated compaction ratio, KV-Surgeon substantially advances the cost--accuracy Pareto frontier of dense and mixture-of-experts models from 4B to 30B parameters. At $50\times$ compaction, KV-Surgeon improves question-answering accuracy by up to four points over attention matching (Zweiger et al., 2026), the state of the art, at comparable cost. Lastly, we introduce an even faster variant, which also exceeds the state of the art while requiring only two fifths of its cost.

==> fig_forest_slope.tex <==
\begin{figure}[t]
  \centering
  \pgfplotsset{
    forest panel/.style={
      width=0.30\linewidth, height=6.2cm,
      xmin=-3, ymin=-1.6, ymax=7.7,
      xlabel={Margin (points)},
      xtick={0,4,8,12}, xmax=12,
      grid=none,
      tick label style={font=\scriptsize},
      yticklabel style={font=\scriptsize, align=right},
      label style={font=\small},
      title style={font=\small},
      axis y line*=left, axis x line*=bottom,
      ytick style={draw=none},
      clip=false,
    },
    frow/.style={color=cobs!60!black, only marks, mark size=1.7pt,
                 error bars/error bar style={color=cobs!60!black, line width=0.6pt},
                 error bars/error mark options={rotate=90, mark size=1.2pt}},
    fpool/.style={color=cobs!60!black, fill=cobs!60!black, mark=none, line width=0.8pt},
  }
  \begin{tikzpicture}[baseline=(current bounding box.north)]
    \begin{axis}[
      forest panel,
      title={KV-Surgeon $-$ AM-HAK},
      ytick={7,6,5,4,3,2,1,-0.55},
      yticklabels={Qwen3-4B / QuAL.,Qwen3-4B / LongH.,Llama-3.1-8B / QuAL.,Llama-3.1-8B / LongH.,Gemma-3-12B / QuAL.,Gemma-3-12B / LongH.,Qwen3-30B-A3B / QuAL.,{\textbf{pooled}}},
    ]
      \addplot[gray!70, thick, forget plot, mark=none] coordinates {(0,-1.5) (0,7.8)};
      \draw[gray!40] (axis cs:-3,0.4) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},0.4);
      \addplot[frow, mark=*] plot[error bars/.cd, x dir=both, x explicit] coordinates {
        (3.42,7.17) +- (0.98,0)
        (5.45,6.17) +- (2.20,0)
        (3.31,5.17) +- (2.48,0)
        (5.60,4.17) +- (2.85,0)
        (3.96,3.17) +- (1.50,0)
        (3.65,2.17) +- (3.68,0)
        (4.14,1.17) +- (1.77,0)
      };
      \addplot[frow, mark=o] plot[error bars/.cd, x dir=both, x explicit] coordinates {
        (2.73,6.83) +- (3.30,0)
        (2.85,5.83) +- (3.32,0)
        (1.90,4.83) +- (1.56,0)
        (3.85,3.83) +- (2.02,0)
        (2.42,2.83) +- (2.70,0)
        (3.70,1.83) +- (3.69,0)
        (3.00,0.83) +- (1.86,0)
      };
      \addplot[fpool] coordinates {(3.35,-0.2) (4.22,0.02) (5.09,-0.2) (4.22,-0.42) (3.35,-0.2)};
      \addplot[fpool, fill=none] coordinates {(2.29,-0.9) (2.92,-0.68) (3.55,-0.9) (2.92,-1.12) (2.29,-0.9)};
      \node[font=\scriptsize, anchor=west, text=cobs!60!black] at (axis cs:5.39,-0.2) {$+4.2$};
      \node[font=\scriptsize, anchor=west, text=cobs!60!black] at (axis cs:3.85,-0.9) {$+2.9$};
    \end{axis}
  \end{tikzpicture}\hspace{-1.2em}
  \begin{tikzpicture}[baseline=(current bounding box.north)]
    \begin{axis}[
      forest panel,
      title={KV-Surgeon $-$ LOO}, xmax=16, xtick={0,4,8,12,16}, xlabel={},
      ytick={7,6,5,4,3,2,1,-0.55},
      yticklabels={},
      yticklabels={},
    ]
      \addplot[gray!70, thick, forget plot, mark=none] coordinates {(0,-1.5) (0,7.8)};
      \draw[gray!40] (axis cs:-3,0.4) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},0.4);
      \addplot[frow, mark=*] plot[error bars/.cd, x dir=both, x explicit] coordinates {
        (1.83,7.17) +- (1.36,0)
        (5.55,6.17) +- (1.96,0)
        (2.35,5.17) +- (2.36,0)
        (9.40,4.17) +- (5.55,0)
        (4.99,3.17) +- (1.36,0)
        (5.80,2.17) +- (4.39,0)
        (2.95,1.17) +- (1.43,0)
      };
      \addplot[frow, mark=o] plot[error bars/.cd, x dir=both, x explicit] coordinates {
        (1.21,6.83) +- (0.75,0)
        (3.70,5.83) +- (3.37,0)
        (1.07,4.83) +- (2.76,0)
        (3.00,3.83) +- (2.16,0)
        (2.39,2.83) +- (2.25,0)
        (6.75,1.83) +- (3.39,0)
        (2.95,0.83) +- (1.86,0)
      };
      \addplot[fpool] coordinates {(2.28,-0.2) (4.70,0.02) (7.11,-0.2) (4.70,-0.42) (2.28,-0.2)};
      \addplot[fpool, fill=none] coordinates {(1.25,-0.9) (3.01,-0.68) (4.78,-0.9) (3.01,-1.12) (1.25,-0.9)};
      \node[font=\scriptsize, anchor=west, text=cobs!60!black] at (axis cs:7.41,-0.2) {$+4.7$};
      \node[font=\scriptsize, anchor=west, text=cobs!60!black] at (axis cs:5.08,-0.9) {$+3.0$};
    \end{axis}
  \end{tikzpicture}\hfill
  \begin{tikzpicture}[baseline=(current bounding box.north)]
    \begin{axis}[
      width=0.34\linewidth, height=6.2cm,
      xmode=log, log basis x=10,
      xmin=4, xmax=130, ymin=-1, ymax=8.5,
      ytick={0,2,4,6,8},
      xtick={5,10,20,50,100}, xticklabels={$5\times$,$10\times$,$20\times$,$50\times$,$100\times$},
      xticklabel style={rotate=45, anchor=north east, inner sep=1pt},
      minor tick num=0,
      x dir=reverse,
      xlabel={Compaction ratio},
      ylabel={Margin (points)},
      tick label style={font=\scriptsize},
      label style={font=\small},
      title style={font=\small},
      title={KV-Surgeon margin against ratio},
      grid=none,
      legend style={font=\scriptsize, at={(0.5,-0.34)}, anchor=north, draw=none, fill=none},
      legend cell align=left,
      legend columns=2,
      every mark/.append style={solid},
      mark size=1.6pt,
    ]
      \draw[gray!60] (axis cs:4,0) -- (axis cs:130,0);
      \addplot[cam, solid, line width=1.1pt, mark=pentagon*, error bars/.cd, y dir=both, y explicit, error bar style={solid, line width=0.6pt, color=cam}] coordinates {(94.0,4.22) +- (0,0.36) (47.0,2.92) +- (0,0.26) (18.8,1.27) +- (0,0.40) (9.4,0.67) +- (0,0.22) (4.7,0.79) +- (0,0.48)};
      \addlegendentry{AM-HAK}
      \addplot[cloo, solid, line width=1.1pt, mark=*, error bars/.cd, y dir=both, y explicit, error bar style={solid, line width=0.6pt, color=cloo}] coordinates {(106.0,4.70) +- (0,0.98) (53.0,3.01) +- (0,0.72) (21.2,1.68) +- (0,0.64) (10.6,0.95) +- (0,0.30) (5.3,0.65) +- (0,0.24)};
      \addlegendentry{LOO}
      \addplot[cam, dashed, line width=1.1pt, mark=pentagon, error bars/.cd, y dir=both, y explicit, error bar style={solid, line width=0.6pt, color=cam}] coordinates {(88.0,6.97) +- (0,1.37) (44.0,7.07) +- (0,1.27) (17.6,2.64) +- (0,0.99) (8.8,0.59) +- (0,0.87) (4.4,0.71) +- (0,0.80)};
      \addlegendentry{AM-HAK-fast}
    \end{axis}
  \end{tikzpicture}
  \caption{Per-combination view of the margins of KV-Surgeon over LOO and AM-HAK in \cref{tab:main-acc}. Left and center: the two controlled comparisons at $100\times$ and
  $50\times$. Each row is one model and benchmark combination; filled
  markers are $100\times$ ($\rho=0.01$), open markers are $50\times$
  ($\rho=0.02$). Bars are $95\%$ intervals of the seed-paired difference
  ($t_4$ over five seeds; unpaired for Qwen3-30B against AM-HAK at $50\times$).
  Diamonds are the mean margin over the seven combinations with its $95\%$
  $t_6$ interval. Every one of the 28 differences is positive. Four of the
  fourteen per-combination intervals against AM-HAK and two against LOO cross
  zero, and the seven-combination means do not. Right: the same two mean margins
  across the full ratio grid (solid) and the corresponding margin in the fast calibration tier,
  KV-Surgeon-fast against AM-HAK-fast (dashed). Bars are one standard
  error over the seven combinations. The margin decays from four points at $100\times$ to noise
  by $10\times$, and does not shrink when the calibration queries get cheap.}
  \label{fig:forest-slope}
\end{figure}


==> fig_surrogate.tex <==
\begin{figure}[t]
  \centering
  \pgfplotsset{
    surr panel/.style={
      width=0.31\linewidth, height=5.4cm,
      tick label style={font=\scriptsize},
      label style={font=\small},
      title style={font=\small},
      grid=none,
      every mark/.append style={solid},
      mark size=1.5pt,
      legend style={font=\scriptsize, draw=none, fill=none, at={(0.5,-0.24)}, anchor=north, /tikz/every even column/.append style={column sep=0.3em}},
      legend cell align=left,
    },
  }
  \begin{tikzpicture}[baseline=(current bounding box.north), trim axis right]
    \begin{axis}[surr panel,
      xmode=log, ymode=log, x dir=reverse,
      xmin=0.007, xmax=1.3, ymin=0.003, ymax=3,
      xtick={1,0.5,0.2,0.1,0.05,0.02,0.01},
      xticklabels={$1$,$.5$,$.2$,$.1$,$.05$,$.02$,$.01$},
      ytick={0.01,0.1,1}, yticklabels={$0.01$,$0.1$,$1$},
      xlabel={Fraction of keys kept},
      ylabel={Ratio},
      title={Surrogate / exact loss},
      legend columns=2,
    ]
      \draw[gray!60] (axis cs:0.007,1) -- (axis cs:1.3,1);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.95,0.659) -- (axis cs:0.95,1.965);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.9,0.713) -- (axis cs:0.9,1.814);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.8,0.766) -- (axis cs:0.8,1.662);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.5,0.645) -- (axis cs:0.5,1.181);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.2,0.318) -- (axis cs:0.2,0.648);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.1,0.18) -- (axis cs:0.1,0.457);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.05,0.096) -- (axis cs:0.05,0.334);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.02,0.04) -- (axis cs:0.02,0.242);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.01,0.021) -- (axis cs:0.01,0.198);
      \addplot[cobs!80!black, solid, line width=0.9pt, mark=triangle*] coordinates {(0.95,1.181) (0.9,1.172) (0.8,1.132) (0.5,0.871) (0.2,0.452) (0.1,0.291) (0.05,0.187) (0.02,0.112) (0.01,0.084)};
      \addlegendentry{surrogate (Qwen)}
      \draw[cloo, line width=0.5pt] (axis cs:0.95,0.096) -- (axis cs:0.95,0.426);
      \draw[cloo, line width=0.5pt] (axis cs:0.9,0.077) -- (axis cs:0.9,0.32);
      \draw[cloo, line width=0.5pt] (axis cs:0.8,0.061) -- (axis cs:0.8,0.25);
      \draw[cloo, line width=0.5pt] (axis cs:0.5,0.043) -- (axis cs:0.5,0.194);
      \draw[cloo, line width=0.5pt] (axis cs:0.2,0.032) -- (axis cs:0.2,0.18);
      \draw[cloo, line width=0.5pt] (axis cs:0.1,0.029) -- (axis cs:0.1,0.171);
      \draw[cloo, line width=0.5pt] (axis cs:0.05,0.024) -- (axis cs:0.05,0.161);
      \draw[cloo, line width=0.5pt] (axis cs:0.02,0.02) -- (axis cs:0.02,0.144);
      \draw[cloo, line width=0.5pt] (axis cs:0.01,0.018) -- (axis cs:0.01,0.126);
      \addplot[cloo, solid, line width=0.9pt, mark=*] coordinates {(0.95,0.216) (0.9,0.157) (0.8,0.122) (0.5,0.097) (0.2,0.076) (0.1,0.063) (0.05,0.053) (0.02,0.042) (0.01,0.035)};
      \addlegendentry{score~\eqref{eq:loo} (Qwen)}
      \addplot[black!45, solid, line width=0.7pt, mark=none] coordinates {(0.5,0.0109) (0.2,0.0914) (0.1,0.2163) (0.05,0.4121) (0.02,0.7105) (0.01,0.9261)};
      \addlegendentry{exact (Qwen)}
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.95,0.668) -- (axis cs:0.95,1.258);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.9,0.761) -- (axis cs:0.9,1.255);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.8,0.791) -- (axis cs:0.8,1.19);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.5,0.586) -- (axis cs:0.5,0.794);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.2,0.228) -- (axis cs:0.2,0.352);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.1,0.1) -- (axis cs:0.1,0.186);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.05,0.043) -- (axis cs:0.05,0.096);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.02,0.014) -- (axis cs:0.02,0.038);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.01,0.006) -- (axis cs:0.01,0.019);
      \addplot[cobs!80!black, dashed, line width=0.9pt, mark=triangle] coordinates {(0.95,0.961) (0.9,1.011) (0.8,0.98) (0.5,0.686) (0.2,0.28) (0.1,0.134) (0.05,0.062) (0.02,0.022) (0.01,0.01)};
      \addlegendentry{surrogate (Llama)}
      \draw[cloo, line width=0.5pt] (axis cs:0.95,0.067) -- (axis cs:0.95,0.317);
      \draw[cloo, line width=0.5pt] (axis cs:0.9,0.057) -- (axis cs:0.9,0.24);
      \draw[cloo, line width=0.5pt] (axis cs:0.8,0.045) -- (axis cs:0.8,0.194);
      \draw[cloo, line width=0.5pt] (axis cs:0.5,0.031) -- (axis cs:0.5,0.145);
      \draw[cloo, line width=0.5pt] (axis cs:0.2,0.023) -- (axis cs:0.2,0.124);
      \draw[cloo, line width=0.5pt] (axis cs:0.1,0.02) -- (axis cs:0.1,0.105);
      \draw[cloo, line width=0.5pt] (axis cs:0.05,0.017) -- (axis cs:0.05,0.088);
      \draw[cloo, line width=0.5pt] (axis cs:0.02,0.013) -- (axis cs:0.02,0.066);
      \draw[cloo, line width=0.5pt] (axis cs:0.01,0.01) -- (axis cs:0.01,0.051);
      \addplot[cloo, dashed, line width=0.9pt, mark=o] coordinates {(0.95,0.17) (0.9,0.137) (0.8,0.104) (0.5,0.071) (0.2,0.053) (0.1,0.042) (0.05,0.034) (0.02,0.025) (0.01,0.019)};
      \addlegendentry{score~\eqref{eq:loo} (Llama)}
      \addplot[black!45, dashed, line width=0.7pt, mark=none] coordinates {(0.5,0.0184) (0.2,0.1311) (0.1,0.3058) (0.05,0.5702) (0.02,1.1) (0.01,1.694)};
      \addlegendentry{exact (Llama)}
    \end{axis}
  \end{tikzpicture}\hfill
  \begin{tikzpicture}[baseline=(current bounding box.north), trim axis left, trim axis right]
    \begin{axis}[surr panel,
      width=0.27\linewidth,
      xmin=-0.6, xmax=2.6, ymin=0, ymax=1.02,
      xtick={0,1,2}, xticklabels={calib., held-out, cheap},
      xticklabel style={rotate=25, anchor=north east, inner sep=1pt},
      ytick={0,0.25,0.5,0.75,1},
      ylabel={Spearman vs.\ exact},
      title={Ranking of deletion sets},
      legend columns=3,
      axis x line*=bottom, axis y line*=left, clip=false,
    ]
      \draw[cobs!80!black, line width=0.5pt] (axis cs:-0.29,0.714) -- (axis cs:-0.29,0.976);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.71,0.357) -- (axis cs:0.71,0.881);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:1.71,0.524) -- (axis cs:1.71,0.929);
      \addplot[cobs!80!black, only marks, mark=triangle*] coordinates {(-0.29,0.905) (0.71,0.69) (1.71,0.786)};
      \addlegendentry{surrogate}
      \draw[cobs!80!black, line width=0.5pt] (axis cs:-0.19,0.786) -- (axis cs:-0.19,0.976);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:0.81,0.357) -- (axis cs:0.81,0.81);
      \draw[cobs!80!black, line width=0.5pt] (axis cs:1.81,0.595) -- (axis cs:1.81,0.952);
      \addplot[cobs!80!black, only marks, mark=triangle] coordinates {(-0.19,0.929) (0.81,0.643) (1.81,0.833)};
      \draw[cloo, line width=0.5pt] (axis cs:-0.05,0.667) -- (axis cs:-0.05,0.976);
      \draw[cloo, line width=0.5pt] (axis cs:0.95,0.262) -- (axis cs:0.95,0.81);
      \draw[cloo, line width=0.5pt] (axis cs:1.95,0.405) -- (axis cs:1.95,0.857);
      \addplot[cloo, only marks, mark=*] coordinates {(-0.05,0.881) (0.95,0.595) (1.95,0.69)};
      \addlegendentry{score~\eqref{eq:loo}}
      \draw[cloo, line width=0.5pt] (axis cs:0.05,0.667) -- (axis cs:0.05,0.952);
      \draw[cloo, line width=0.5pt] (axis cs:1.05,0.19) -- (axis cs:1.05,0.738);
      \draw[cloo, line width=0.5pt] (axis cs:2.05,0.405) -- (axis cs:2.05,0.857);
      \addplot[cloo, only marks, mark=o] coordinates {(0.05,0.881) (1.05,0.524) (2.05,0.69)};
      \draw[black!55, line width=0.5pt] (axis cs:0.19,0.571) -- (axis cs:0.19,0.929);
      \draw[black!55, line width=0.5pt] (axis cs:1.19,0.333) -- (axis cs:1.19,0.833);
      \draw[black!55, line width=0.5pt] (axis cs:2.19,0.405) -- (axis cs:2.19,0.881);
      \addplot[black!55, only marks, mark=square*] coordinates {(0.19,0.81) (1.19,0.643) (2.19,0.714)};
      \addlegendentry{diagonal}
      \draw[black!55, line width=0.5pt] (axis cs:0.29,0.595) -- (axis cs:0.29,0.929);
      \draw[black!55, line width=0.5pt] (axis cs:1.29,0.31) -- (axis cs:1.29,0.786);
      \draw[black!55, line width=0.5pt] (axis cs:2.29,0.429) -- (axis cs:2.29,0.857);
      \addplot[black!55, only marks, mark=square] coordinates {(0.29,0.81) (1.29,0.595) (2.29,0.714)};
    \end{axis}
  \end{tikzpicture}\hfill
  \begin{tikzpicture}[baseline=(current bounding box.north), trim axis left]
    \begin{axis}[surr panel,
      width=0.27\linewidth,
      xmode=log, xmin=0.003, xmax=1.6, ymin=0, ymax=1.02,
      xtick={0.01,0.1,1}, xticklabels={$0.01$,$0.1$,$1$},
      ytick={0,0.25,0.5,0.75,1},
      xlabel={Exact loss / raw eviction},
      ylabel={Fraction of heads},
      title={Compensation, $50\times$},
      legend columns=2,
    ]
      \draw[gray!60] (axis cs:1,0) -- (axis cs:1,1.02);
      \addplot[cobs!80!black, solid, line width=1.0pt, mark=none] coordinates {(0.00549,0.000) (0.01986,0.017) (0.02474,0.033) (0.03001,0.050) (0.0356,0.067) (0.04068,0.083) (0.04394,0.100) (0.04936,0.117) (0.05416,0.133) (0.05941,0.150) (0.06528,0.167) (0.06915,0.183) (0.07486,0.200) (0.08102,0.217) (0.0898,0.233) (0.09589,0.250) (0.1027,0.267) (0.112,0.283) (0.124,0.300) (0.1312,0.317) (0.1401,0.333) (0.1518,0.350) (0.1653,0.367) (0.1739,0.383) (0.1882,0.400) (0.1985,0.417) (0.2074,0.433) (0.2145,0.450) (0.2276,0.467) (0.2392,0.483) (0.2513,0.500) (0.2649,0.517) (0.2781,0.533) (0.2875,0.550) (0.2966,0.567) (0.3093,0.583) (0.3174,0.600) (0.3286,0.617) (0.3369,0.633) (0.3473,0.650) (0.3544,0.667) (0.3641,0.683) (0.373,0.700) (0.3812,0.717) (0.3942,0.733) (0.4067,0.750) (0.4183,0.767) (0.4278,0.783) (0.434,0.800) (0.4473,0.817) (0.4627,0.833) (0.4759,0.850) (0.491,0.867) (0.5064,0.883) (0.5266,0.900) (0.5471,0.917) (0.5718,0.933) (0.6009,0.950) (0.6303,0.967) (0.683,0.983) (1.174,1.000)};
      \addlegendentry{final refit (Qwen)}
      \addplot[black!55, solid, line width=0.8pt, mark=none] coordinates {(0.006827,0.000) (0.01949,0.017) (0.02653,0.033) (0.0313,0.050) (0.03706,0.067) (0.04246,0.083) (0.04572,0.100) (0.05086,0.117) (0.05674,0.133) (0.06161,0.150) (0.06661,0.167) (0.07184,0.183) (0.07606,0.200) (0.08351,0.217) (0.09374,0.233) (0.1024,0.250) (0.1097,0.267) (0.1242,0.283) (0.1342,0.300) (0.1468,0.317) (0.1565,0.333) (0.1792,0.350) (0.1933,0.367) (0.2131,0.383) (0.2285,0.400) (0.243,0.417) (0.2572,0.433) (0.2695,0.450) (0.279,0.467) (0.2948,0.483) (0.3114,0.500) (0.3242,0.517) (0.3391,0.533) (0.353,0.550) (0.3649,0.567) (0.3863,0.583) (0.3992,0.600) (0.4127,0.617) (0.4225,0.633) (0.4309,0.650) (0.4407,0.667) (0.4476,0.683) (0.4565,0.700) (0.4712,0.717) (0.4853,0.733) (0.506,0.750) (0.5179,0.767) (0.5301,0.783) (0.5446,0.800) (0.5561,0.817) (0.5718,0.833) (0.5875,0.850) (0.6037,0.867) (0.622,0.883) (0.6409,0.900) (0.6643,0.917) (0.6995,0.933) (0.7364,0.950) (0.7956,0.967) (0.9198,0.983) (2.578e+10,1.000)};
      \addlegendentry{elimination (Qwen)}
      \addplot[cobs!80!black, dashed, line width=1.0pt, mark=none] coordinates {(0.003881,0.000) (0.01301,0.017) (0.01717,0.033) (0.01971,0.050) (0.02123,0.067) (0.02301,0.083) (0.02463,0.100) (0.02639,0.117) (0.02749,0.133) (0.02869,0.150) (0.03025,0.167) (0.03169,0.183) (0.03276,0.200) (0.03438,0.217) (0.03584,0.233) (0.03733,0.250) (0.03915,0.267) (0.04078,0.283) (0.04269,0.300) (0.04557,0.317) (0.04775,0.333) (0.05012,0.350) (0.05221,0.367) (0.0548,0.383) (0.05808,0.400) (0.06049,0.417) (0.06327,0.433) (0.06597,0.450) (0.0699,0.467) (0.07194,0.483) (0.07484,0.500) (0.07771,0.517) (0.07976,0.533) (0.08139,0.550) (0.08429,0.567) (0.08713,0.583) (0.08921,0.600) (0.09403,0.617) (0.0986,0.633) (0.1027,0.650) (0.1063,0.667) (0.1099,0.683) (0.1138,0.700) (0.1181,0.717) (0.122,0.733) (0.1294,0.750) (0.1345,0.767) (0.1393,0.783) (0.1464,0.800) (0.1543,0.817) (0.1643,0.833) (0.1729,0.850) (0.1875,0.867) (0.2104,0.883) (0.2346,0.900) (0.2602,0.917) (0.2775,0.933) (0.3095,0.950) (0.3585,0.967) (0.4186,0.983) (0.8668,1.000)};
      \addlegendentry{final refit (Llama)}
      \addplot[black!55, dashed, line width=0.8pt, mark=none] coordinates {(0.004522,0.000) (0.01303,0.017) (0.01648,0.033) (0.01958,0.050) (0.02135,0.067) (0.02306,0.083) (0.02442,0.100) (0.0259,0.117) (0.02758,0.133) (0.02872,0.150) (0.03021,0.167) (0.03208,0.183) (0.03354,0.200) (0.03467,0.217) (0.03658,0.233) (0.03823,0.250) (0.0404,0.267) (0.04258,0.283) (0.04547,0.300) (0.04882,0.317) (0.05074,0.333) (0.0529,0.350) (0.05526,0.367) (0.05792,0.383) (0.06178,0.400) (0.06514,0.417) (0.06914,0.433) (0.07287,0.450) (0.07582,0.467) (0.07724,0.483) (0.08035,0.500) (0.08358,0.517) (0.08645,0.533) (0.08971,0.550) (0.0931,0.567) (0.0972,0.583) (0.101,0.600) (0.1041,0.617) (0.1084,0.633) (0.1135,0.650) (0.1191,0.667) (0.1214,0.683) (0.1293,0.700) (0.136,0.717) (0.1447,0.733) (0.1517,0.750) (0.1608,0.767) (0.1739,0.783) (0.1807,0.800) (0.1966,0.817) (0.2146,0.833) (0.2338,0.850) (0.2547,0.867) (0.2731,0.883) (0.2957,0.900) (0.3474,0.917) (0.4217,0.933) (2.246e+06,0.950) (3.013e+08,0.967) (2.046e+09,0.983) (3.279e+10,1.000)};
      \addlegendentry{elimination (Llama)}
    \end{axis}
  \end{tikzpicture}
  \caption{The surrogate chain measured on queries it never saw: scores computed
  from self-study calibration queries, exact loss evaluated on held-out benchmark
  questions, Qwen3-4B (Qwen; solid, filled) and Llama-3.1-8B (Llama; dashed, open), five
  QuALITY articles, every head (1440 and 1280 head--article pairs). Left: the
  surrogate of \cref{eq:decoupled0} and the additive score of \cref{eq:loo} as a
  fraction of the exact loss along the LOO ranking, median and inter-quartile
  range over heads, with the exact loss relative to $\lVert O\rVert_F^2$ in gray.
  Center: Spearman correlation between surrogate and exact loss over random
  subsets of the candidate pool, computed within one head and one set size (never
  pooled across sizes), median and inter-quartile range over $20{,}160$ and $17{,}920$
  groups; \emph{calib.} evaluates the exact loss on the calibration queries,
  \emph{held-out} on benchmark questions, \emph{cheap} recomputes the scores from
  a single repeat pass. Right: on the supports KV-Surgeon actually selects at
  $50\times$, the exact held-out loss of the stored cache relative to raw eviction
  of the same keys, as a cumulative distribution over heads, for the final refit
  of \cref{sec:refit} and for the coefficients the elimination itself produces;
  the elimination curves leave the plot to the right on the $1\%$ and $5\%$ of heads
  where those coefficients diverge.}
  \label{fig:surrogate}
\end{figure}

